The Governance of Intimacy: A Preliminary Policy Analysis of Romantic AI Platforms

Romantic AI platforms invite intimate emotional disclosure, yet their data governance practices remain underexamined. This preliminary study analyses the Privacy Policies and Terms of Service of six Western and Chinese romantic AI platforms. We find that intimate disclosures are often positioned as reusable data assets, with broad permissions for storage, analysis, and model training. We identify default training appropriation, ownership reconstruction, and intimate history assetization as key mechanisms structuring these practices, expanding platforms' rights while shifting risk onto users. Our findings surface key governance challenges in romantic AI and are intended to provoke discussion and inform future empirical and design research on human AI intimacy and its governance.

==> archieve.tex <==
\section{Introduction}

We aim to address the following research questions:



\begin{enumerate}
    \item[\textbf{RQ1}:] How do romantic AI partner platforms describe their data practices — including collection, usage, disclosure/sharing — and, where applicable, their AI-specific governance (e.g., disclaimers, content restrictions, ownership of outputs, liability) in their privacy policies and terms of service?
    \item[\textbf{RQ2}:] Which stakeholders are acknowledged in romantic AI platform policies, and how clearly are their rights and responsibilities defined?
    \item[\textbf{RQ3}:] How do these policies align with international data protection frameworks and ethical AI guidelines?

\end{enumerate}



We could use PoliAnalyze~\cite{zhao2025let} to conduct a large-scale and comprehensive automatic analysis of romantic apps.



